Incremental Multimodal Surface Mapping via Self-Organizing Gaussian Mixture Models

This letter describes an incremental multimodal surface mapping methodology, which represents the environment as a continuous probabilistic model. This model enables high-resolution reconstruction while simultaneously compressing spatial and intensity point cloud data. The strategy employed in this work utilizes Gaussian mixture models (GMMs) to represent the environment. While prior GMM-based mapping works have developed methodologies to determine the number of mixture components using information-theoretic techniques, these approaches either operate on individual sensor observations, making them unsuitable for incremental mapping, or are not real-time viable, especially for applications where high-fidelity modeling is required. To bridge this gap, this letter introduces a spatial hash map for rapid GMM submap extraction combined with an approach to determine relevant and redundant data in a point cloud. These contributions increase computational speed by an order of magnitude compared to state-of-the-art incremental GMM-based mapping. In addition, the proposed approach yields a superior tradeoff in map accuracy and size when compared to state-of-the-art mapping methodologies (both GMM- and not GMM-based). Evaluations are conducted using both simulated and real-world data. The software is released open-source to benefit the robotics community.

==> content/figure_containers/psnr_mre_variation_plots.tex <==
% \begin{figure}
%   \centering
%   \subfloat{\input{figures/psnr_0_0135.tex}}%
%   \subfloat{\input{figures/mre_0_0135.tex}}
%   \caption{\label{fig:psnr-image-size}Variation of PSNR (left) and MRE (right)
%   with image sizes for a fixed $\sigma = 0.0135$ on Ryzen/RTX3090. The reconstruction
%   accuracy varies monotonically with the image size when the bandwidth is fixed.}
% \end{figure}

\begin{figure*}
  \centering
  \subfloat{\includegraphics[width=0.5\linewidth]{figures/psnr_0_0135_raincloud.eps}}%
  \subfloat{\includegraphics[width=0.5\linewidth]{figures/mre_0_0135_raincloud.eps}}%
  \caption{\label{fig:psnr-image-size}Variation of PSNR (left) and MRE (right)
  with image sizes for a fixed $\sigma = 0.0135$ on Ryzen/RTX3090. Empirically, the reconstruction
  accuracy varies monotonically with the image size when the bandwidth is fixed.}
\end{figure*}

==> content/figure_containers/reconstruction_plots.tex <==

\begin{figure*}
  % \captionsetup[subfigure]{labelformat=empty}
  \centering
  \begin{minipage}{0.25\textwidth}
    \centering
    \subfloat[Ryzen/RTX3090, \SI{0.9}{\second}, $M = 267$]{\label{sfig:103-rtx3090}\includegraphics[width=\textwidth,trim=420 125 420 125,clip]{figures/eps/rtx3090/recon_103_RTX3090.eps}}\\
    \subfloat[Ryzen/RTX3090, \SI{1.9}{\second}, $M = 459$]{\label{sfig:2364-rtx3090}\includegraphics[width=\textwidth,trim=420 125 420 125,clip]{figures/eps/rtx3090/recon_2364_RTX3090.eps}}\\
    \subfloat[Ryzen/RTX3090, \SI{2.6}{\second}, $M = 601$]{\label{sfig:4173-rtx3090}\includegraphics[width=\textwidth,trim=420 125 420 125,clip]{figures/eps/rtx3090/recon_4173_RTX3090.eps}}\\
    \subfloat[Ryzen/RTX3090, \SI{8.2}{\second}, $M = 655$]{\label{sfig:935-rtx3090}\includegraphics[width=\textwidth,trim=420 125 420 125,clip]{figures/eps/rtx3090/recon_935_RTX3090.eps}}\\
    \subfloat[Ryzen/RTX3090, \SI{6.5}{\second}, $M = 710$]{\label{sfig:1763-rtx3090}\includegraphics[width=\textwidth,trim=420 125 420 125,clip]{figures/eps/rtx3090/recon_1763_RTX3090.eps}}
  \end{minipage}%
  \begin{minipage}{0.25\textwidth}
    \centering
    \subfloat[Ryzen/RTX3060, \SI{1.0}{\second}, $M = 254$]{\label{sfig:103-rtx3060}\includegraphics[width=\textwidth,trim=420 125 420 125,clip]{figures/eps/rtx3060/recon_103_RTX3060.eps}}\\
    \subfloat[Ryzen/RTX3060, \SI{2.2}{\second}, $M = 463$]{\label{sfig:2364-rtx3060}\includegraphics[width=\textwidth,trim=420 125 420 125,clip]{figures/eps/rtx3060/recon_2364_RTX3060.eps}}\\
    \subfloat[Ryzen/RTX3060, \SI{2.6}{\second}, $M = 392$]{\label{sfig:4173-rtx3060}\includegraphics[width=\textwidth,trim=420 125 420 125,clip]{figures/eps/rtx3060/recon_4173_RTX3060.eps}}\\
    \subfloat[Ryzen/RTX3060, \SI{5.9}{\second}, $M = 716$]{\label{sfig:935-rtx3060}\includegraphics[width=\textwidth,trim=420 125 420 125,clip]{figures/eps/rtx3060/recon_935_RTX3060.eps}}\\
    \subfloat[Ryzen/RTX3060, \SI{7.1}{\second}, $M = 412$]{\label{sfig:1763-rtx3060}\includegraphics[width=\textwidth,trim=420 125 420 125,clip]{figures/eps/rtx3060/recon_1763_RTX3060.eps}}
  \end{minipage}%
  \begin{minipage}{0.25\textwidth}
    \centering
    \subfloat[ARM-12c/Orin, \SI{2.8}{\second}, $M = 106$]{\label{sfig:103-orin}\includegraphics[width=\textwidth,trim=420 125 420 125,clip]{figures/eps/orin/recon_103_Orin.eps}}\\
    \subfloat[ARM-12c/Orin, \SI{4.3}{\second}, $M = 212$]{\label{sfig:2364-orin}\includegraphics[width=\textwidth,trim=420 125 420 125,clip]{figures/eps/orin/recon_2364_Orin.eps}}\\
    \subfloat[ARM-12c/Orin, \SI{5.3}{\second}, $M = 269$]{\label{sfig:4173-orin}\includegraphics[width=\textwidth,trim=420 125 420 125,clip]{figures/eps/orin/recon_4173_Orin.eps}}\\
    \subfloat[ARM-12c/Orin, \SI{5.8}{\second}, $M = 320$]{\label{sfig:935-orin}\includegraphics[width=\textwidth,trim=420 125 420 125,clip]{figures/eps/orin/recon_935_Orin.eps}}\\
    \subfloat[ARM-12c/Orin, \SI{6.7}{\second}, $M = 336$]{\label{sfig:1763-orin}\includegraphics[width=\textwidth,trim=420 125 420 125,clip]{figures/eps/orin/recon_1763_Orin.eps}}
  \end{minipage}%
  \begin{minipage}{0.25\textwidth}
    \centering
    \subfloat[ARM-8c/Xavier, \SI{2.0}{\second}, $M = 55$]{\label{sfig:103-xavier}\includegraphics[width=\textwidth,trim=420 125 420 125,clip]{figures/eps/xavier/recon_103_Xavier.eps}}\\
    \subfloat[ARM-8c/Xavier, \SI{4.0}{\second}, $M = 100$]{\label{sfig:2364-xavier}\includegraphics[width=\textwidth,trim=420 125 420 125,clip]{figures/eps/xavier/recon_2364_Xavier.eps}}\\
    \subfloat[ARM-8c/Xavier, \SI{4.4}{\second}, $M = 124$]{\label{sfig:4173-xavier}\includegraphics[width=\textwidth,trim=420 125 420 125,clip]{figures/eps/xavier/recon_4173_Xavier.eps}}\\
    \subfloat[ARM-8c/Xavier, \SI{6.7}{\second}, $M = 278$]{\label{sfig:935-xavier}\includegraphics[width=\textwidth,trim=420 125 420 125,clip]{figures/eps/xavier/recon_935_Xavier.eps}}\\
    \subfloat[ARM-8c/Xavier, \SI{6.9}{\second}, $M = 280$]{\label{sfig:1763-xavier}\includegraphics[width=\textwidth,trim=420 125 420 125,clip]{figures/eps/xavier/recon_1763_Xavier.eps}}
  \end{minipage}%
  \caption{\label{fig:H5-qual}Reconstruction outputs for the scenes shown in~\cref{fig:real-data}
  using the parameters corresponding to the highest PSNR values
  in~\cref{fig:H5-quant}.
  \protect\subref{sfig:103-rtx3090}--\protect\subref{sfig:1763-rtx3090} show the
  results for the Ryzen/RTX3090 platform.
  \protect\subref{sfig:103-rtx3060}--\protect\subref{sfig:1763-rtx3060} show the
  results for the Ryzen/RTX3060 platform.
  \protect\subref{sfig:103-orin}--\protect\subref{sfig:1763-orin} show the
  results for the ARM-12c/Orin platform.
  \protect\subref{sfig:103-xavier}--\protect\subref{sfig:1763-xavier} show the
  results for the ARM-8c/Xavier platform. Choosing the lowest possible bandwidth
  and highest possible image size might provide better reconstruction results at
  a cost of high fit times, as done in~\citep{goel_probabilistic_2023}. In
  contrast, setting the image size and the bandwidth parameters together
  informed through time budget and available compute
  (e.g.,~\cref{stab:five-sec}) allows an approximate tradeoff in the number of
  components, the SOGMM fit time, and the reconstruction quality across scenes
  with varying depth and intensity complexity.
  }
\end{figure*}


==> content/figure_containers/scene_plots.tex <==
\begin{figure*}
  \centering
  \subfloat[I1]{\label{sfig:103-gt}\includegraphics[width=0.2\textwidth,trim=420 125 420 125,clip]{figures/eps/pcd_stonewall_103_decimate_1_0.eps}}%
  \subfloat[I2]{\label{sfig:2364-gt}\includegraphics[width=0.2\textwidth,trim=420 125 420 125,clip]{figures/eps/pcd_copyroom_2364_decimate_1_0.eps}}%
  \subfloat[I3]{\label{sfig:4173-gt}\includegraphics[width=0.2\textwidth,trim=420 125 420 125,clip]{figures/eps/pcd_copyroom_4173_decimate_1_0.eps}}%
  \subfloat[I4]{\label{sfig:935-gt}\includegraphics[width=0.2\textwidth,trim=420 125 420 125,clip]{figures/eps/pcd_copyroom_935_decimate_1_0.eps}}%
  \subfloat[I5]{\label{sfig:1763-gt}\includegraphics[width=0.2\textwidth,trim=420 125 420 125,clip]{figures/eps/pcd_lounge_1763_decimate_1_0.eps}}
  \caption{\label{fig:real-data}(Left to right) Scenes of increasing depth and intensity complexity from
    the ICL-NUIM datasets~\citep{zhou_dense_2013}, used for evaluating~\ref{H5} and~\ref{H6}.}
\end{figure*}


==> content/figure_containers/sogmm_computation_time_plots.tex <==
\begin{figure*}
  \centering
  \subfloat[\label{sfig:rtx3090-sogmm}Ryzen/RTX3090, SOGMM]{\input{figures/rtx3090-sogmm.tex}}%
  \subfloat[\label{sfig:rtx3060-sogmm}Intel/RTX3060, SOGMM]{\input{figures/rtx3060-sogmm.tex}}%
  \subfloat[\label{sfig:orin-sogmm}ARM-12c/Orin, SOGMM]{\input{figures/orin-sogmm.tex}}\\
  \subfloat[\label{sfig:xavier-sogmm}ARM-8c/Xavier, SOGMM]{\input{figures/xavier-sogmm.tex}}
  \subfloat[\label{sfig:tx2-sogmm}ARM-6c/TX2, SOGMM]{\input{figures/tx2-sogmm.tex}}
  \subfloat[\label{sfig:ryzen-scikit}Comparison with \texttt{scikit-learn} on Ryzen]{\input{figures/ryzen-scikit.tex}}\\
  \subfloat[\label{stab:five-sec}Cases where SOGMM fit time is less than or equal to \SI{5}{\second}]{\input{figures/five_seconds_table.tex}}%
  \caption{\label{fig:sogmm-compute}
    Comparison of SOGMM computation time on the target platforms listed
    in~\cref{tab:targets}. In~\protect\subref{sfig:rtx3090-sogmm}
    and~\protect\subref{sfig:rtx3060-sogmm} the GPU-accelerated case
      on the desktop platforms provides more than an order of magnitude improvement
      in timing compared to the CPU-only case for most image sizes.
     The results of the embedded platforms shown in \protect\subref{sfig:orin-sogmm},~\protect\subref{sfig:xavier-sogmm}
     and~\protect\subref{sfig:tx2-sogmm} demonstrate that the relative performance improvements seem to
     degrade with increasing SWaP constraints.
    In any case,~\protect\subref{sfig:ryzen-scikit} shows that our CPU implementation performs
    nearly an order of magnitude faster than a reference SOGMM implementation
    using \texttt{scikit-learn}.~\protect\subref{stab:five-sec} lists the
    cases where the fit took less than or equal to \SI{5}{\second}.}
\end{figure*}


==> content/figure_containers/sogmm_fit_times_iclnuim.tex <==
\begin{figure*}
  \centering
  \begin{minipage}{0.25\textwidth}
    \centering
    \subfloat{\input{figures/times_RTX3090.tex}}\\
    \addtocounter{subfigure}{-1}
    \subfloat{\input{figures/psnr_RTX3090.tex}}\\
    \addtocounter{subfigure}{-1}
    \subfloat[Ryzen/RTX3090]{\input{figures/mre_RTX3090.tex}}
  \end{minipage}%
  \begin{minipage}{0.25\textwidth}
    \subfloat{\input{figures/times_RTX3060.tex}}\\
    \addtocounter{subfigure}{-1}
    \subfloat{\input{figures/psnr_RTX3060.tex}}\\
    \addtocounter{subfigure}{-1}
    \subfloat[Intel/RTX3060]{\input{figures/mre_RTX3060.tex}}
  \end{minipage}%
  \begin{minipage}{0.25\textwidth}
    \subfloat{\input{figures/times_Orin.tex}}\\
    \addtocounter{subfigure}{-1}
    \subfloat{\input{figures/psnr_Orin.tex}}\\
    \addtocounter{subfigure}{-1}
    \subfloat[ARM-12c/Orin]{\input{figures/mre_Orin.tex}}
  \vspace{-0.35cm}
  \end{minipage}%
  \begin{minipage}{0.25\textwidth}
    \subfloat{\input{figures/times_Xavier.tex}}\\
    \addtocounter{subfigure}{-1}
    \subfloat{\input{figures/psnr_Xavier.tex}}\\
    \addtocounter{subfigure}{-1}
    \subfloat[ARM-8c/Xavier]{\input{figures/mre_Xavier.tex}}
  \vspace{-0.66cm}
  \end{minipage}
  \caption{\label{fig:H5-quant}
    From top to bottom, row 1 provides the SOGMM fit times,
    row 2 illustrates the PSNR scores, and row 3
      provides MRE scores for the images shown
    in~\cref{fig:real-data}. The bandwidth and image
    sizes for these plots are selected according to the values
      for each device shown in~\cref{stab:five-sec}.
    Each column corresponds to a different device.
    We observe an overall degradation in PSNR
    and MRE scores for all images as the compute capability decreases
    (left to right). All devices output the model in times around but not
    strictly below the \SI{5}{\second} time budget. These
    experiments are used to evaluate~\ref{H5}.}
%(Left to right) For each device in~\cref{tab:targets},
\end{figure*}


==> content/figure_containers/target_platforms_table.tex <==
%% Figures
\begin{table*}[h]
  \centering
  \begin{tabular}{c|cccc}
    \textbf{Platform ID} & \textbf{Platform Type} & \textbf{CPU}                             & \textbf{GPU}            & \textbf{Memory (CPU/GPU)}                \\
    \hline
    % Ryzen/RTX3090        & Desktop                & AMD Ryzen Threadripper 3960X, 48 threads & NVIDIA GeForce RTX 3090 & \SI{252}{\giga\byte}/\SI{24}{\giga\byte} \\
    Intel/RTX3060        & Desktop                & Intel Core i9-10900K, 20 threads         & NVIDIA GeForce RTX 3060 & \SI{32}{\giga\byte}/\SI{12}{\giga\byte}  \\
    ARM-12c/Orin         & Embedded               & ARMv8 Processor rev 1 (v8l), 12 threads  & NVIDIA Jetson Orin      & \SI{32}{\giga\byte}                      \\
    ARM-8c/Xavier        & Embedded               & ARMv8 Processor rev 0 (v8l), 8 threads   & NVIDIA Jetson Xavier    & \SI{16}{\giga\byte}                      \\
    % ARM-6c/TX2           & Embedded               & ARM Cortex-A57, 6 threads                & NVIDIA Jetson TX2       & \SI{8}{\giga\byte}
  \end{tabular}
  \caption{\label{tab:targets}Target platforms used for evaluation.}
\end{table*}


==> content/impl_detail.tex <==
\begin{figure}
  \includegraphics[width=\linewidth]{figures/information_flow.eps}%
  \caption{\label{fig:information-flow}Information flow for the proposed GPU-accelerated adaptive point cloud
  modeling system. Given a depth-intensity image pair and bandwidth, the approach
  runs Gaussian Blurring Mean Shift (GBMS) on the CPU to obtain the number of components $\nComponents$.
  The number of components and the 4D data are used by KInit on the CPU to calculate the initial responsibility
  matrix used by the Expectation Maximization (EM) algorithm on the GPU. The final result from the EM
  algorithm is the SOGMM model~\citep{goel_probabilistic_2023}.}
\end{figure}

This section details GPU-accelerated software architecture of
the SOGMM framework presented in~\citep{goel_probabilistic_2023} and the incremental
mapping method proposed in this work.~\Cref{fig:information-flow} shows an overview of the SOGMM system.
The GBMS and KInit algorithms are implemented on the CPU while the EM algorithm
is accelerated via the GPU.

\subsection{SOGMM Implementation.}
The GBMS algorithm is implemented on the CPU in our
system.~\citet{comaniciu_mean_2002} propose using a binned estimator where the
bins are represented by a grid with cell size equal to the bandwidth parameter
$\sigma$. The positions of these bins are used as seeds for the algorithm. For
each seed, a mechanism is required to query the neighbors in $\datasetY$ within
the grid cell. Because our implementation processes lower-dimensional (i.e., 2D)
data, we leverage a kd-tree~\cite{blanco2014nanoflann} to perform the range
search; however, for higher-dimensional data it may be more efficient to use a
BallTree~\cite{omohundro1989five,pedregosa2011scikit}. The returned points
within the specified radius are averaged and the seed is updated to the new
location. For each seed, the algorithm terminates if the number of maximum
iterations is reached or if there is no substantial change with respect to the
previous seed position.

The EM algorithm consists of two steps: Expectation (E) and Maximization (M).
We reduce the computational complexity of the E step by converting the
multiplications and divisions into sums and differences.
The E Step evaluates the responsibilities $\resp_{nb}$ using the current
parameters $\mean_b$, $\cov_b$ and $\weight_b$ via
\begin{align}
  \resp_{nb} &= \frac{\weight_b \gaussian{\pointx_n}{\mean_b}{\cov_b}{}}
               {\sum\limits_{a=1}^{\nComponents} \weight_a \gaussian{\pointx_n}{\mean_a}{\cov_a}{}}.
               \label{eq:estep}
\end{align}
To reduce the computational complexity of~\cref{eq:estep}, the natural logarithm
can be applied to convert the multiplications and divisions into sums and
differences:
\begin{align}
  \ln \resp_{nb} &= \ln \weight_b + \ln \left( \gaussian{\pointx_n}{\mean_b}{\cov_b}{} \right) \notag \\
                 &~~~~~~~ - \ln \left( \sum\limits_{a=1}^{\nComponents} \weight_a \gaussian{\pointx_n}{\mean_a}{\cov_a}{} \right).
  \label{eq:logestep}
\end{align}
Term 2 of~\cref{eq:logestep} may be rewritten, as derived in~\cite{buitinck2013api,pedregosa2011scikit,wenniethesis},
\begin{footnotesize}
\begin{align}
  &\ln \left( \gaussian{\pointx_n}{\mean_b}{\cov_b}{} \right) \notag\\
  % &=\ln \left( \frac{\exp \left( -\frac{1}{2}(\pointx_n - \mean_b)^{\top} \cov_b^{-1}(\pointx_n - \mean_b) \right)}{(2\pi)^{D/2}|\cov_b|^{1/2}} \right) \notag\\
  % &=\ln \left( \frac{\exp\left( -\frac{1}{2}(\pointx_n - \mean_b)^{\top} \precchol_b^{\top}\precchol_b(\pointx_n - \mean_b)\right)}{(2\pi)^{D/2}|\cov_b|^{1/2}} \right)\notag\\
  % &=-\frac{1}{2}\left( D\ln(2\pi) + \ln(|\cov_b|) + (\pointx_n - \mean_b)^{\top} \precchol_b^{\top}\precchol_b(\pointx_n - \mean_b) \right)\notag\\
  % &=-\frac{1}{2}\left( D\ln(2\pi) + (\pointx_n - \mean_b)^{\top} \precchol_b^{\top}\precchol_b(\pointx_n - \mean_b) \right) + \ln(|\cov_b|^{-1/2})\notag\\
  &=-\frac{1}{2}\left( D\ln(2\pi) + \sum\limits_{j=1}^D \left( \precchol_b(\pointx_n - \mean_b)  \right)_j^2 \right) + \left( \sum_{j=1}^D \ln \left(\text{diag}(\precchol_b)\right)_j \right)
  \label{eq:simplifiedGaussian}
\end{align}
\end{footnotesize}
where $\cov = \lowerL\lowerL^{\top}$, $\precchol = \lowerL^{-1}$, and $\lowerL$ is a
lower triangular matrix calculated using the Cholesky decomposition of the
covariance matrix.  Summing the logarithm of the diagonal entries of
$\precchol_b$ (i.e., $\ln(\text{diag}(\precchol_b))$)
in~\cref{eq:simplifiedGaussian} is equivalent to $\ln|\cov_b|^{-1/2}$.

The GPU implementation leverages higher-order tensor representations (rank-$3$
and rank-$4$ tensors)\footnote{For the exposition of the GPU-accelerated
components, tensor conventions from TensorFlow~\citep{abadi2016tensorflow} are
used.}. The weights are represented as a rank-$3$ tensor of shape $(1,
\nComponents, 1)$, means are represented as a rank-$3$ tensor of shape $(1,
\nComponents, 4)$, and covariances are represented as a rank-$4$ tensor of shape
$(1, \nComponents, 4, 4)$. This implementation accelerates unary (e.g.,
logarithm and exponential of a matrix, reduction operations like
summing along a dimension or taking a maximum along a dimension of a
rank-$2$ or a rank-$3$ tensor) and binary (e.g., addition,
subtraction, multiplication, and division of rank-$2$ and rank-$3$
tensors) operations via element-wise CUDA kernels with fixed block and
grid sizes for all GPUs.

Matrix multiplications of two rank-$2$ tensors are accelerated using the
\texttt{cuBLAS}\footnote{\texttt{cuBLAS} \url{https://docs.nvidia.com/cuda/cublas}}
\texttt{gemm} routine. Matrix multiplications of two rank-$3$ tensors are
accelerated via the \texttt{cuBLAS} \texttt{gemmStridedBatched} routine. The
Cholesky decomposition of a rank-$2$ tensor is accelerated via the
\texttt{cuSOLVER}\footnote{\texttt{cuSOLVER} \url{https://docs.nvidia.com/cuda/cusolver}}
\texttt{potrf} routine.  The Cholesky decomposition of a rank-$3$ tensor is
accelerated using the \texttt{cuSOLVER} \texttt{potrfBatched} routine.  Using
the Cholesky decomposition, a linear system of equations involving rank-$2$
tensors is solved using the \texttt{cuSOLVER} \texttt{potrs} routine and for rank-$3$ tensors using
the \texttt{potrsBatched} routine.

% \subsection{Hash Table Implementation.}

% \subsection{Global Inference Implementation.}
% %% Algorithm for Inference
% \begin{algorithm}
%   \DontPrintSemicolon

%   \SetKwInput{Input}{input}
%   \SetKwInput{Parameters}{parameters}
%   \SetKwInput{Output}{output}

%   \SetKwFunction{EmptyPcld}{EmptyPointCloud}
%   \SetKwFunction{BoxMuller}{BoxMuller}

%   \Input{The global model $\gsogmm$.}
%   \Parameters{Std. deviation $\spatialstddev$, Number of points $| \pointcloud |$.}
%   \Output{Reconstructed 4D point cloud $\pointcloud$.}
%   \BlankLine
%   $\pointcloud \leftarrow \EmptyPcld(| \pointcloud |, 4)$\;
%   \For{$b \in \findexset$}{
%     $| \pointcloud |_b \leftarrow \gweight_b | \pointcloud |$ \tcp*[r]{Points in Gaussian $b$}
%     $\pointcloud(| \pointcloud |_b, 0:3) \leftarrow \BoxMuller( \gsogmm(b), | \pointcloud |_b, \spatialstddev)$\\
%   }
%   \caption{Global Spatial and Intensity Inference}
% \end{algorithm}

% \textbf{Software Package Details.}
% The software is implemented using C++17 and also provides a Python 3.8
% interface via python bindings created using \texttt{pybind11}~\citep{pybind11}.
% The software is compiled using GCC-8 and NVCC (version less than or equal to
% 12.1) for all platforms. Element-wise CUDA kernels from \texttt{Open3D} were
% leveraged to enable easy integration with its point cloud utilities.  The
% framework is built using \texttt{colcon}\footnote{\texttt{colcon}
% \url{https://colcon.readthedocs.io/en/released/}} to enable future integration
% with \texttt{ROS2}~\citep{ros2}.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> content/impl_detail_old.tex <==
\begin{figure}
  \includegraphics[width=\linewidth]{figures/information_flow.eps}%
  \caption{\label{fig:information-flow}Information flow for the proposed GPU-accelerated adaptive point cloud
  modeling system. Given a depth-intensity image pair, desired image size, and bandwidth, the approach
  runs Gaussian Blurring Mean Shift (GBMS) on the CPU to obtain the number of components $\nComponents$.
  The number of components and the 4D data are used by KInit on the CPU to calculate the initial responsibility
  matrix used by the Expectation Maximization (EM) algorithm on the GPU. The final result from the EM
  algorithm is the SOGMM model~\citep{goel_probabilistic_2023}.}
\end{figure}

\red{
\begin{enumerate}
  \item Remove CPU stuff
  \item Remove math background where unnecessary
  \item Focus on GPU impl for EM
  \item Focus on speed up in inference using the hash map
  \item Focus on how to get this to work on platforms with different computational capability
\end{enumerate}
}

This section details the CPU-only and GPU-accelerated software architecture of
the SOGMM framework presented in~\citep{goel_probabilistic_2023}. We
provide background information for the components of the SOGMM framework: the
Gaussian Blurring Mean Shift (GBMS) algorithm, initialization of the Expectation
Maximization (EM) algorithm using the KInit method, and the EM algorithm itself.
Details on how these algorithms are implemented for the CPU-only and the
GPU-accelerated versions of our software system are also provided.

\Cref{fig:information-flow} shows an overview of the proposed software system.
After a depth-intensity image pair is received and resized, the depth and
intensity vectors (i.e., 2D data) are processed by GBMS to estimate the number of
components for KInit and EM algorithms. The KInit algorithm is the first step of
the K-Means++ algorithm, which is detailed in steps (1a)--(1c)
of~\citet{arthur_k-means_2007}. It outputs the posterior probabilities
used by the EM algorithm for initialization. The EM algorithm iteratively finds
a local maximum of the log-likelihood of the data with respect to the GMM model
parameters.

\textbf{Notation.} We follow the notation from~\cite{goel_probabilistic_2023},
which uses small letters for scalars (e.g., $x$, $y$), bolded small letters for
vectors (e.g., $\pointx$, $\pointy$), bolded capital letters for matrices (e.g.,
$\mathbf{X}$, $\mathbf{Y}$), and calligraphic letters for sets (e.g.,
$\imagepair$, $\datasetX$, $\datasetY$). Additionally, for the exposition of the
GPU-accelerated components, tensor
conventions\footnote{\url{https://www.tensorflow.org/guide/tensor}} from
TensorFlow~\citep{abadi2016tensorflow} are used.

\textbf{Gaussian Mixture Model.} A GMM represents multivariate data $(D \in
\mathbb{Z}_{> 0})$ as a weighted combination of $M$ Gaussian densities~\citep[p.
110]{bishop2006pattern}. The probability density function of a GMM is parameterized by a set
$\gmmparams = \{\pi_m, \mean_m, \cov_m \}_{m=1}^M$, where $\weight \in
\mathbb{R}$ is a weight and $\sum_{m} \pi_m = 1$.  The probability
density of the GMM is written as
\begin{align}
  p(\pointx \mid \gmmparams) = \sum_{m=1}^M \weight_m \gaussian{\pointx}{\mean_m}{\cov_m}
  \label{eq:model}
\end{align}
where $\pointx \in \mathbb{R}^D$ is an independent and identically
distributed (i.i.d) sample drawn with distribution $\p$, and
\begin{align}
  \gaussian{\pointx}{\mean_m}{\cov_m}{} = \frac{\exp\left( -\frac{1}{2} (\pointx - \mean_m)^{\top} \cov_m^{-1} (\pointx - \mean_m)\right)}{(2\pi)^{D/2}|\cov_m|^{1/2}}
\end{align}
is the probability density function of a Gaussian distribution with mean $\mean_m
\in \mathbb{R}^{D}$ and covariance $\cov_m \in \mathbb{R}^{D\times D}$.

The parameter set $\gmmparams$ is represented only
with vectors and 2D matrices in the CPU implementation of the proposed
framework while the GPU implementation leverages higher-order tensor
representations (e.g., rank-$3$ tensors).  In the CPU
implementation, weights are represented as a vector
(i.e., rank-$1$ tensor) of shape $(\nComponents)$, means are
represented as a matrix (i.e., rank-$2$ tensor) of shape
$(\nComponents, D)$, and covariances are represented as a
rank-$2$ tensor of shape $(\nComponents, D^2)$.  In the GPU
implementation, weights are represented as a
rank-$3$ tensor of shape $(1, \nComponents, 1)$, means are
represented as a rank-$3$ tensor of shape $(1, \nComponents,
D)$, and covariances are represented as a rank-$4$ tensor of
shape $(1, \nComponents, D, D)$. In the SOGMM framework, $D = 4$ and
$\nComponents$ is decided using the GBMS algorithm.

\textbf{Gaussian Blurring Mean Shift (GBMS).}
To determine $\nComponents$, SOGMM utilizes the GBMS
algorithm~\citep{comaniciu_mean_2002,carreira-perpinan_fast_2006} using the
update rule:
\begin{align}
  \pointy^{t}_{r, i} \leftarrow \frac{ \sumoverkernel{j=1}{|\datasetY|}{\pointy^{t-1}_{r,i}}{\pointy^{t-1}_j} \pointy^{t-1}_j}{\sumoverkernel{j=1}{|\datasetY|}{\pointy^{t-1}_i}{\pointy^{t-1}_j}}.
  \label{eq:gbms}
\end{align}
where
\begin{align}
  \kernel{\pointy - \pointy_i} = \begin{cases} 1 & \text{if } \| \pointy - \pointy_i \| \leq \sigma \\ 0 &\text{if } \| \pointy - \pointy_i \| > \sigma \end{cases}
  \label{eq:flatkernel}
\end{align}
is the flat kernel and $\pointy \in \mathbb{R}^2$ consists of the raw depth and intensity
values. The bandwidth parameter is denoted by $\sigma$.  Note that $|\datasetY| =
|\datasetX|$ where $\datasetX$ is the four-dimensional point cloud consisting of
the 3D data with the intensity values in the fourth dimension.

This algorithm is implemented on the CPU in our
system.~\citet{comaniciu_mean_2002} propose using a binned estimator
where the bins are represented by a grid with cell size equal to the
bandwidth parameter $\sigma$. The positions of these bins are used as
seeds for the algorithm. For each seed, a mechanism is required to
query the neighbors in $\datasetY$ within the grid
cell. Because our implementation processes lower-dimensional
(i.e., 2D) data, we leverage a kd-tree~\cite{blanco2014nanoflann} to
perform the range search; however, for higher-dimensional data it may
be more efficient to use a
BallTree~\cite{omohundro1989five,pedregosa2011scikit}. The returned
points within the specified radius are averaged and the seed is
updated to the new location.  For each seed, the algorithm terminates
if the number of maximum iterations is reached or
if there is no substantial change with respect to the previous seed
position.

\textbf{Expectation Maximization Initialization (KInit).} To initialize Expectation
Maximization, $\nComponents$ clusters must be selected. The result of this
initialization step are tuples of centers and indices $(\cluster_{\componentid},
j)$, where $j \in \{1, \dots, | \datasetX | \}$.

These indices are used to initialize the matrix of posterior
probabilities, also known as the \emph{responsibility matrix} for the
Expectation Maximization
algorithm~\citep[p.112]{bishop2006pattern}. The responsibility matrix
$\Resp^1 \in \mathbb{R}^{\nSamples \times \nComponents}$ with entries
$\resp_{n'm'}$, where $n' \in \{1, \ldots, |\datasetX|\}$ and $m' \in
\{1, \dots, M\}$, is initialized using the tuples
$(\cluster_{\componentid}, j)$ according to the following formula:
\begin{align}
\resp^1_{n'm'} =
     \begin{cases}
       \text{1.0,} &\quad \text{if } n' = j \text{ and } m' = m\\
       \text{0.0,} &\quad \text{otherwise} \\
     \end{cases}
\end{align}
The initialized responsibility matrix $\Resp^1$, updated with the M step, is
updated in successive iterations of EM using the superscript $i$, (i.e.,
$\Resp^i$).

\textbf{Expectation Maximization (EM).} The objective of the EM algorithm is to
find the GMM parameters $\gmmparams^*$ that maximize the likelihood
$\likelihood$ that the dataset $\datasetX$ was sampled from the
  probability density function in~\cref{eq:model}:
\begin{align}
  \gmmparams^* &= \arg\max\limits_{\gmmparams} \ln{\likelihoodfun{\gmmparams}{\datasetX}} \notag\\
  &= \arg\max\limits_{\gmmparams} \ln{ \left( \prod\limits_{n=1}^N p(\pointx_n|\gmmparams) \right) } \notag\\
  &= \arg\max\limits_{\gmmparams} \sum\limits_{n=1}^N \ln{ \left( p(\pointx_n|\gmmparams) \right) } \notag\\
  &= \arg\max\limits_{\gmmparams} \sum\limits_{n=1}^N \ln{ \left( \sum_{m=1}^M \weight_m \gaussian{\pointx_n}{\mean_m}{\cov_m} \right).}
  \label{eq:max-likeli}
\end{align}
The presence of the summation over $m$ inside the logarithm
in~\cref{eq:max-likeli} makes the solution for $\gmmparams$ impossible to
compute analytically~\citep[p.113]{bishop2006pattern}. The EM algorithm provides
an iterative scheme to find the locally optimal solution for this problem.
It consists of two steps: the Expectation (E) step and the Maximization (M) step.

The E Step evaluates the responsibilities $\resp_{nm}$ using the current
parameters $\mean_m$, $\cov_m$ and $\weight_m$ via
\begin{align}
  \resp_{nm} &= \frac{\weight_m \gaussian{\pointx_n}{\mean_m}{\cov_m}{}}
               {\sum\limits_{j=1}^{\nComponents} \weight_j \gaussian{\pointx_n}{\mean_j}{\cov_j}{}}.
               \label{eq:estep}
\end{align}
To reduce the computational complexity of~\cref{eq:estep}, the natural logarithm can be applied
to convert the multiplications and divisions into sums and
differences:
\begin{align}
  \ln \resp_{nm} &= \ln \weight_m + \ln \left( \gaussian{\pointx_n}{\mean_m}{\cov_m}{} \right) \notag \\
                 &~~~~~~~ - \ln \left( \sum\limits_{j=1}^{\nComponents} \weight_j \gaussian{\pointx_n}{\mean_j}{\cov_j}{} \right).
  \label{eq:logestep}
\end{align}
Term 2 of~\cref{eq:logestep} may be rewritten as~\cite{buitinck2013api,pedregosa2011scikit,wenniethesis}:
\begin{footnotesize}
\begin{align}
  &\ln \left( \gaussian{\pointx_n}{\mean_m}{\cov_m}{} \right) \notag\\
  &=\ln \left( \frac{\exp \left( -\frac{1}{2}(\pointx_n - \mean_m)^{\top} \cov_m^{-1}(\pointx_n - \mean_m) \right)}{(2\pi)^{D/2}|\cov_m|^{1/2}} \right) \notag\\
  &=\ln \left( \frac{\exp\left( -\frac{1}{2}(\pointx_n - \mean_m)^{\top} \precchol_m^{\top}\precchol_m(\pointx_n - \mean_m)\right)}{(2\pi)^{D/2}|\cov_m|^{1/2}} \right)\notag\\
  &=-\frac{1}{2}\left( D\ln(2\pi) + \ln(|\cov_m|) + (\pointx_n - \mean_m)^{\top} \precchol_m^{\top}\precchol_m(\pointx_n - \mean_m) \right)\notag\\
  &=-\frac{1}{2}\left( D\ln(2\pi) + (\pointx_n - \mean_m)^{\top} \precchol_m^{\top}\precchol_m(\pointx_n - \mean_m) \right) + \ln(|\cov_m|^{-1/2})\notag\\
  &=-\frac{1}{2}\left( D\ln(2\pi) + \sum\limits_{j=1}^D \left( \precchol_m(\pointx_n - \mean_m)  \right)_j^2 \right) + \left( \sum_{j=1}^D \ln \left(\text{diag}(\precchol_m)\right)_j \right)
  \label{eq:simplifiedGaussian}
\end{align}
\end{footnotesize}
where
\begin{align}
  \cov &= \lowerL\lowerL^{\top}\notag\\
  \precchol &= \lowerL^{-1}
  \label{eq:cholesky}
\end{align}
and $\lowerL$ in~\cref{eq:cholesky} is a lower triangular matrix calculated
using the Cholesky decomposition of the covariance matrix.  Summing the logarithm of the
diagonal entries of $\precchol_m$ (i.e., $\ln(\text{diag}(\precchol_m))$)
in~\cref{eq:simplifiedGaussian} is equivalent to $\ln|\cov_m|^{-1/2}$.

In the CPU implementation of~\cref{eq:logestep}, the dataset $\datasetX$ is a
rank-$2$ tensor of shape $(N, D)$ and the responsibility matrix $\Resp$ is a
rank-$2$ tensor of shape $(N, \nComponents)$. The first two terms
of~\cref{eq:logestep} are summed and the resulting matrix is used to calculate
the third term.

The M step updates the means, covariances, and weights
using the responsibility matrix calculated in~\cref{eq:estep}
\begin{align}
  \weight_m^* &=  \sum\limits_{n=1}^N \resp_{nm} \label{eq:save_compute}\\
  \mean_m^{i+1} &= \sum\limits_{n=1}^N \frac{\resp_{nm}\pointx_n}{\weight^*_m} \label{eq:mstep_means}\\
  \cov_m^{i+1} &= \sum\limits_{n=1}^N \frac{(\pointx_n - \mean_m^{i+1})(\pointx_n - \mean_m^{i+1})^{\top} \resp_{nm}}{\pi_m^*} \label{eq:mstep_covs}\\
  \pi_m^{i+1} &= \frac{\pi_m^*}{N} \label{eq:mstep_weights}
\end{align}
\Cref{eq:save_compute} stores the sum of the responsibilities without
normalization for efficient calculation of the means and covariances.

The GPU implementation accelerates unary (e.g.,
logarithm and exponential of a matrix, reduction operations like
summing along a dimension or taking a maximum along a dimension of a
rank-$2$ or a rank-$3$ tensor) and binary (e.g., addition,
subtraction, multiplication, and division of rank-$2$ and rank-$3$
tensors) operations via element-wise CUDA kernels with fixed block and
grid sizes for all GPUs.

Matrix multiplications of two rank-$2$ tensors are accelerated using the
\texttt{cuBLAS}\footnote{\texttt{cuBLAS} \url{https://docs.nvidia.com/cuda/cublas/index.html}}
\texttt{gemm} routine. Matrix multiplications of two rank-$3$ tensors are
accelerated via the \texttt{cuBLAS} \texttt{gemmStridedBatched} routine. The
Cholesky decomposition of a rank-$2$ tensor is accelerated via the
\texttt{cuSOLVER}\footnote{\texttt{cuSOLVER} \url{https://docs.nvidia.com/cuda/cusolver/}}
\texttt{potrf} routine.  The Cholesky decomposition of a rank-$3$ tensor is
accelerated using the \texttt{cuSOLVER} \texttt{potrfBatched} routine.  Using
the Cholesky decomposition, a linear system of equations involving rank-$2$
tensors is solved using the \texttt{cuSOLVER} \texttt{potrs} routine and for rank-$3$ tensors using
the \texttt{potrsBatched} routine.

The software was implemented using C++17 and also provides a Python 3.8
interface via python bindings created using \texttt{pybind11}~\citep{pybind11}.  The
software was compiled using GCC-8 and NVCC v11.4 for all platforms except the
NVIDIA Jetson TX2, which used NVCC v10.2.  Element-wise CUDA kernels from \texttt{Open3D}
were leveraged to enable easy integration with its point cloud utilities.
The framework
is built using \texttt{colcon}\footnote{\texttt{colcon} \url{https://colcon.readthedocs.io/en/released/}}
to enable future integration with \texttt{ROS2}~\citep{ros2}.


==> content/isomath.tex <==
\newcommand*{\fontsetup}{\usepackage%
% {ae}%             \sfdefault is cmss
% {anttor}%         \sfdefault is cmss (use iwona)
% {arev}%           normal and sans identic (also in math)
% {beton}%          bitmap fonts
% {concmath}%
% {cmbright}%
% {fourier}%        incompatible (uses private font encoding)
% [default]{gfsneohellenic}% no bold
% {hfoldsty}%       bitmap fonts
% {iwona}%          sets cmss as sans font (use iwona)
% [nomathscript]{kpfonts}% "Too many math alphabets" with OMLmathsfit option
% {kerkis}%         no bold math,
% {lmodern}%        \sfdefault is cmss
% {lucidabr}%       commercial, subset (no math) free as bitmap
% {lxfonts}%        normal and sans identic,
[utopia]{mathdesign}% \sfdefault is cmss, provides roman and roman-bold in OML
% [charter]{mathdesign}%
% [garamond]{mathdesign}%
% {mathptmx}%       in mathnormal, Greek is larger than Latin!
% {mbtimes}%        \sfdefault is cmss
% {mathpazo}%       \sfdefault is cmss
% {newcent}%        \sfdefault is cmss
% {pxfonts}%        needs reuseMathAlphabets, no sans-serif
% {tgcursor}%       avoid bitmap tt
% {tgheros}%        avoid bitmap sf
% {tgpagella}%      \sfdefault is cmss
% {tgtermes}%       \sfdefault is cmss
% {txfonts}%        no sans-serif
}

% Isomath setup
% ~~~~~~~~~~~~~
%
% Uncomment the option(s) you want to test ::

\newcommand*{\isomathsetup}{\usepackage[%
% reuseMathAlphabets,%
OMLmathrm,%
OMLmathbf,%
% OMLmathsf,%
% OMLmathsfit,%
% OMLmathtt,%
% OMLmathsans,% backwards compatibility option alias
% rmdefault=zpple,% Mathpazo alternative
% rmdefault=qtxmia,% TeX Gyre Termes math with alternative glyphs
% sfdefault=cmbr,%   default
% sfdefault=iwona,%  Iwona sans (Greek glyphs too close to roman)
sfdefault=fav,%    Arev sans (scale down (ca. 0.87))
scaled=0.875%      scaling for Arev (small letters)
% sfdefault=llcmss,% LX sans (glyphs too close to italic, scale down)
% sfdefault=jkpss,%   Kepler Sans
% scaled=0.95%      scaling for Kepler Sans (small letters)
]{isomath}%
}

% Load customisable packages
% --------------------------
% ::

\fontsetup
\isomathsetup

% Auxiliary definitions
% ---------------------
%
% Re-define \vec to comply with ISO 31::

\renewcommand*{\vec}{\vectorsym}

% Fall-back definition for \mathsfit::

\providecommand*{\mathsfit}[1]%
{\emph{mathsfit not defined (requires \texttt{OMLmathsfit} option)}}


% use Arev as "heavy" sans serif font::

\DeclareFontShape{OML}{fav}{bx}{it}{<-> s * [0.875] zavmbi7m}{}
\SetMathAlphabet{\mathsfbfit}{bold}{OML}{fav}{bx}{it}

\newcommand{\teststring}{%
% capital Latin letters
A,B,C,
% capital Greek letters
\Gamma,\Delta,\Theta,\Lambda,\Xi,\Pi,\Sigma,\Upsilon,\Phi,\Psi,\Omega,
% small Greek letters
\alpha,\beta,\pi,\nu,\omega,
% small Latin letters:
% compare \nu, \omega, v, and w
v,w,
% is there a true italic form of a and g?
a,g,
% digits
0,1,9
}

\DeclareMathAlphabet{\mathcall}{OMS}{cmsy}{m}{n}


==> content/legacy/evaluation.tex <==
\input{content/figure_containers/target_platforms_table}
\input{content/figure_containers/sogmm_computation_time_plots}

\input{content/figure_containers/scene_plots}
\input{content/figure_containers/sogmm_fit_times_iclnuim}
\input{content/figure_containers/reconstruction_plots}
\input{content/figure_containers/psnr_mre_variation_plots}

%% Text
The proposed framework is evaluated using publicly available
datasets~\citep{zhou_dense_2013} on two desktop and three embedded platforms.
Details of the hardware configurations for these platforms are provided
in~\cref{tab:targets}. The choice of target platform is motivated by
the following considerations:
  (1) embedded GPUs are leveraged in multi-robot teams~\citep{tranzatto_cerberus_2022,agha_nebula_2022,goel_rapid_2021},
  (2) desktop GPUs are popular in works that leverage and improve upon
  NeRFs~\citep{mildenhall_nerf_2020,rosinol_nerf-slam_2022} for training,
  testing, and rendering;
  (3) the platforms vary widely in processing capability; and
  (4) the platforms vary widely in the available memory,
which enables experimentation under incremental memory constraints.

\textbf{Performance Measures.} The computation time is
the total time taken from the timestamp when the SOGMM system receives the
depth-intensity image pair to the timestamp when the GMM is created successfully
(i.e., total time includes GBMS, KInit, and EM). These timestamps are
measured using the
\texttt{std::chrono}\footnote{\texttt{std::chrono} \url{https://en.cppreference.com/w/cpp/header/chrono}}
library on the CPU. The EM implementation is ported to the GPU for
the GPU-accelerated cases. Mean Shift and KInit are on the
CPU for both cases in all the experiments. The accuracy measures for point cloud
reconstruction are the same as in~\citep{goel_probabilistic_2023}: Peak-Signal-to-Noise
Ratio (PSNR) and Mean Reconstruction Error (MRE) between the ground truth and the
reconstructed point clouds. These quantities are computed using
\texttt{scikit-image}~\citep{scikit-image} and
\texttt{Open3D}~\citep{zhou2018open3d} respectively. Note that ground truth
point clouds are fixed in image size at $640 \times 480$ while the reconstructed
point clouds of the same size can be obtained using SOGMMs created from smaller
image sizes.

\textbf{Experimental Setup \& Results.} Experiments are designed
to test the following hypotheses:
\begin{enumerate}[label=\textbf{H\arabic*},start=1]
  \item \label{H1} The GPU-accelerated SOGMM system outperforms the CPU-only version in terms of computation time on
        all target platforms.
  \item \label{H2} The CPU-only SOGMM system outperforms
        a reference implementation of SOGMM that utilizes the \texttt{MeanShift}\footnote{\url{https://scikit-learn.org/stable/modules/generated/sklearn.cluster.MeanShift.html}},
        \texttt{kmeans\_plusplus}\footnote{\url{https://scikit-learn.org/stable/modules/generated/sklearn.cluster.kmeans_plusplus.html}},
        and \texttt{GaussianMixture}\footnote{\url{https://scikit-learn.org/stable/modules/generated/sklearn.mixture.GaussianMixture.html}}
        objects from \texttt{scikit-learn}~\citep{pedregosa2011scikit} in terms of computation time.
  \item \label{H3} Decreasing the bandwidth parameter increases computation time.
  \item \label{H4} Increasing the image size increases computation time.
  \item \label{H5} The bandwidth parameter and image size can be set based on a specific time budget.
  \item \label{H6} Increasing the image size increases point cloud reconstruction accuracy.
\end{enumerate}

\textbf{Evaluation of \ref{H1}:} To evaluate the first hypothesis, an ablation
study is conducted. The time taken to compute a SOGMM is studied as a function
of bandwidth parameter for the platforms outlined in~\cref{fig:sogmm-compute}.
The input data for this experiment corresponds
to frame 854, which was randomly selected, of the
simulated \texttt{livingroom1} data from the Augmented ICL-NUIM
datasets~\citep{zhou_dense_2013}. Ten equally spaced bandwidth values
from $0.0135$ to $0.0300$ are used.  Image sizes of $320 \times 240$,
$213 \times 160$, and $160 \times 120$ are used (corresponding to $2
\times$, $3 \times$, and $4 \times$ reduction along each axis of the
original $640 \times 480$ image). Because there is randomness
in the KInit step, each case is run ten times and averaged to obtain
accurate timing results.

\Cref{sfig:rtx3090-sogmm,sfig:rtx3060-sogmm,sfig:orin-sogmm,sfig:xavier-sogmm,sfig:tx2-sogmm}
plot the results of these trials for the CPU-only (dashed
lines with triangle markers) and GPU-accelerated (solid lines with
circle markers) implementations. Note that the y-axes of these plots
use a base-10 log-scale and the observed standard deviation,
which is plotted as error bars, is very low compared to the mean
values. From~\cref{sfig:rtx3090-sogmm,sfig:rtx3060-sogmm} we observe
over an order of magnitude faster performance when using the
GPU-accelerated version of the system for all image sizes. Further,
there is an overall decrease in performance from Ryzen/RTX3090
(\cref{sfig:rtx3090-sogmm}) to Intel/RTX3060
(\cref{sfig:rtx3060-sogmm}) for both CPU-only and GPU-accelerated
versions. This is expected due to the decrease in computational
capability for both the CPU and GPU.

\Cref{sfig:orin-sogmm} provides results for
ARM-12c/Orin platform. In this case, the gains for the GPU-accelerated version
are lower than the desktop platforms. Notice that for image size $320 \times
240$ the CPU starts performing better than GPU at low bandwidths. At low
bandwidths, the number of estimated components are high.

\Cref{sfig:xavier-sogmm,sfig:tx2-sogmm} suggest a further decrease in relative
performance improvement in using the GPU-accelerated version as opposed to the CPU-only
version of our system. Further, due to memory constraints the $320 \times 240$
image size fails for both platforms below certain bandwidths. Both ARM-8c/Xavier
and ARM-6c/TX2 are SWaP-constrained platforms used on robots.
For real-world usage of our framework, we recommend using the CPU-only
version when CPU resources are not required by other subsystems (e.g., planning,
control, and visual-inertial odometry) and using the GPU-accelerated version
when CPU resources are in demand (which is often the case). The hypothesis
\ref{H1} is false for these platforms.

\textbf{Evaluation of \ref{H2}:} \Cref{sfig:ryzen-scikit} performs the
same analysis as the other plots in~\cref{fig:sogmm-compute}
but compares the performance of the Ryzen/RTX3090 CPU-only
version (bold lines) against a Python implementation from
\texttt{scikit-learn}, which does not use GPU acceleration. We
observe close to an order of magnitude of reduction in computation
time across all bandwidths and image sizes with the output GMM
parameters being equal up to $3$ decimal places. Therefore,
hypothesis \ref{H2} is true.

\textbf{Evaluation of \ref{H3}:} It is clear
from~\cref{fig:sogmm-compute} that the variation in the SOGMM
computation time is not strictly monotonic with respect to the
bandwidth parameter. Therefore, the hypothesis \ref{H3} is false.

\textbf{Evaluation of \ref{H4}:} In~\cref{fig:sogmm-compute} we
observe a strict increase in computation time due to increase in image
size, so the hypothesis \ref{H4} is true. This is expected due to the
increase in the number of points being processed.

\textbf{Evaluation of \ref{H5}:} To test hypothesis \ref{H5}, we leverage
insights from \ref{H1}, \ref{H3}, and \ref{H4} to select a bandwidth value
according to a fixed time budget. We select \SI{5}{\second} since it provides
sufficient bandwidth variation for the platforms under consideration.
To obtain answers for hypothesis \ref{H5}, we design an experiment
that applies the bandwidth under all the same conditions (i.e., the last two
columns of~\cref{stab:five-sec}) but different input data. The new input data
comes from three scenes from the ICL-NUIM datasets~\citep{zhou_dense_2013}: (1)
\texttt{stonewall} (\cref{sfig:103-gt}), (2) \texttt{copyroom}
(\cref{sfig:2364-gt,sfig:4173-gt,sfig:935-gt}), and (3) \texttt{lounge}
(\cref{sfig:1763-gt}).  If the hypothesis holds, the time should be close to
\SI{5}{\second}.  If the hypothesis fails, the time should be significantly more
or less than \SI{5}{\second}. \Cref{fig:H5-quant} shows the timing,
PSNR, and MRE results for this experiment. From the timing results it is clear
that \ref{H5} does not hold because the times tend to increase according to the
environment complexity (i.e., higher number of components calculated for the
same bandwidth). An area of future work is to enable point cloud modeling under
a fixed time budget. For a qualitative analysis of the reconstruction,
the cases corresponding to the highest PSNR values for each device are
visualized in~\cref{fig:H5-qual}. The objective is to understand how well the
timing analysis translates if we fix the bandwidth and image size while varying
the input data. Because the desktop-grade hardware can process more data than
the embedded systems given the same time, the bandwidth and image size
parameters were selected to optimize for time as opposed to reconstruction
quality. This difference in reconstruction quality is clear when comparing the
output of the Ryzen/RTX3090 to the ARM-8c/Xavier, for example. This analysis is
critical for real-time robotic systems that must achieve a given rate in order
to remain safe or complete a task within the required time.

\textbf{Evaluation of \ref{H6}:} \Cref{fig:psnr-image-size} shows the variation
of PSNR and MRE with image size while keeping the bandwidth fixed to its lowest
value used in our analysis $\sigma = 0.0135$. As expected, the PSNR and MRE
vary monotonically with the image size. This is because in the case of larger image sizes,
the SOGMM model is trained on a larger number of points and thus provides a better fit
with respect to the original image pair. Thus, the hypothesis \ref{H6} is true.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:

